Comparing Knowledge Sources for Open-Domain Scientific Claim Verification

The increasing rate at which scientific knowledge is discovered and health claims shared online has highlighted the importance of developing efficient fact-checking systems for scientific claims. The usual setting for this task in the literature assumes that the documents containing the evidence for claims are already provided and annotated or contained in a limited corpus. This renders the systems unrealistic for real-world settings where knowledge sources with potentially millions of documents need to be queried to find relevant evidence. In this paper, we perform an array of experiments to test the performance of open-domain claim verification systems. We test the final verdict prediction of systems on four datasets of biomedical and health claims in different settings. While keeping the pipeline's evidence selection and verdict prediction parts constant, document retrieval is performed over three common knowledge sources (PubMed, Wikipedia, Google) and using two different information retrieval techniques. We show that PubMed works better with specialized biomedical claims, while Wikipedia is more suited for everyday health concerns. Likewise, BM25 excels in retrieval precision, while semantic search in recall of relevant evidence. We discuss the results, outline frequent retrieval patterns and challenges, and provide promising future directions.

==> dump.tex <==
%%OLD TABLE
\iffalse
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htpb]
\small
\centering
\begin{tabular}{p{24mm} p{62mm} p{62mm} }
\hline
\textbf{Example claim  }      & \textbf{Knowledge Source \#1  }         & \textbf{Knowledge Source \#2   }     \\ \hline
(\textsc{SciFact}) & \textit{PubMed (Dense) }    & \textit{PubMed (Sparse)} \\
\textbf{A deficiency of vitamin B12 decreases blood levels of homocysteine.} (\textbf{\textcolor{red}{Refuted}})                    & Lower levels of the three water-soluble vitamins--folate, vitamin b6 and vitamin b12--are primary determinants of high blood homocysteine levels. (...) Recent studies focusing on the reduction of plasma homocysteine as a risk factor for vascular disease showed that vitamin b(6) reduces plasma folate levels. (\textbf{\textcolor{teal}{Supported}})                &    Twelve (63\%) of the 19 vitamin b12-deficient patients had elevated total homocysteine levels. (...) We conclude that there is a significant association of deficiencies of hb, iron, folic acid, and vitamin b12 and abnormally high blood homocysteine level with olp. (\textbf{\textcolor{red}{Refuted}})           \\
                     &                    &                 \\
  (\textsc{PubMedQA})  & \textit{Wikipedia (Dense) } & \textit{PubMed (Dense)}  \\
  \textbf{Does psychological distress predict disability?} (\textbf{\textcolor{teal}{Supported}})              & Mental distress can potentially lead to a change of behavior, affect a person's emotions in a negative way, and affect their relationships with the people around them. People under constant distress are more likely to become sick, mentally or physically. (\textbf{\textcolor{teal}{Supported}})                 &  The results of the mediation analysis suggest that approximately 30\% of the relationship between subacute pain and later disability is dependent on the level of patients' psychological distress. The finding that psychological distress only partially (30\%) mediated the pain-disability relationship indicates that other factors should also be explored.      (\textbf{\textcolor{red}{Refuted}})          \\
                     &                    &                 \\
(\textsc{HealthFC})   & \textit{Wikipedia (Sparse)} & \textit{Google snippets}  \\
\textbf{Does regular consumption of coffee increase the risk of heart disease such as heart attack or stroke?}     (\textbf{\textcolor{red}{Refuted}})                &    Drinking more than this amount actually increases the risk of heart disease, high blood pressure, atrial fibrillation, and stroke. (...) There is an increased risk of hypertriglyceridemia, cardiomyopathy, hypertension, and stroke if three or more standard drinks of alcohol are taken per day.       (\textbf{\textcolor{teal}{Supported}})         &         A meta-analysis concluded that coffee consumption did not provided any prophylactic effect on cardiovascular diseases but did not pose an increased risk either[...] \/\/ | The cohort study data suggest very little excess risk of coronary heart disease among habitual coffee drinkers. The case-controled data[...]   (\textbf{\textcolor{red}{Refuted}})    \\ 
                     &                    &                 \\
 (\textsc{CoVert})  & \textit{Alpaca (7B) } & \textit{Med-Alpaca (7B) }\\
 \textbf{Covid causes heart inflammation in like 70\% of people (including asymptomatic).  That seems like a high rate of heart inflammation!} (\textbf{\textcolor{red}{Refuted}})   &    Yes, the claim is true. According to research, approximately 70\% of people with COVID-19 may develop inflammation of the heart, even if they do not have any symptoms of the virus. This is because the virus can cause long-term damage to the heart even if the person appears to be healthy.    (\textbf{\textcolor{teal}{Supported}})          &      No, the claim is not true. Heart inflammation (myocarditis) is a rare condition that can be caused by a variety of factors, including viral infections. However, studies have found that the rate of myocarditis in patients with COVID-19 is similar to that seen in patients with other respiratory infections, such as the flu. While myocarditis can be a serious condition, it is not seen in the majority of patients with COVID-19. (\textbf{\textcolor{red}{Refuted}}) \\ \hline

          
\end{tabular}
\caption{\label{tab:comparison} Example claims and retrieved evidence from two different knowledge sources, or using two different retrieval techniques, where only one of them provided a correct final verdict.}
\end{table*}

%%%%
\fi


\iffalse
%ALPACA
\begin{table*}[htpb]
\centering
%\resizebox{\textwidth}{!}
{
\def\arraystretch{1.3}
\begin{tabular}{c|ccc|ccc}
\hline
\multicolumn{1}{l}{} & \multicolumn{3}{c}{\textbf{Alpaca (7B)}} & \multicolumn{3}{c}{\textbf{Med-Alpaca (7B)}} \\ \hline
\textbf{Dataset} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 Score} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 Score} \\ \hline
\textsc{SciFact} & $67.6$ & $76.9$ & $72.0$ & $68.2$ & $90.3$ & $77.7$ \\
\textsc{PubMedQA} & $67.5$ & $66.2$ & $66.9$ & $66.3$ & $92.6$ & $77.3$ \\ 
\textsc{HealthFC} & $63.5$ & $73.3$ & $68.0$ & $62.6$ & $78.7$ & $69.7$ \\
\textsc{CoVert} & $76.7$ & $64.1$ & $69.8$ & $73.8$ & $85.3$ & $79.2$ \\
\end{tabular}

}
\caption{\label{tab:llms}Results of final verdict prediction over four datasets using evidence generated by LLMs.}
\end{table*}
\fi

\iffalse
%% WIDE TABLE

\begin{table*}[htpb]
\small
\centering
\begin{tabular}{p{20mm} p{125mm} }
\hline
\textbf{Example claim  }      & \textbf{Knowledge }     \\ \hline
(\textsc{SciFact}) & \textit{PubMed (Dense) }    \textit{PubMed (Sparse)} \\
Claim & \textbf{A deficiency of vitamin B12 decreases blood levels of homocysteine.} (\textbf{\textcolor{red}{Refuted}})          \\
Evidence 1 & \textit{Lower levels of the three water-soluble vitamins--folate, vitamin b6 and vitamin b12--are primary determinants of high blood homocysteine levels. (...) Recent studies focusing on the reduction of plasma homocysteine as a risk factor for vascular disease showed that vitamin b(6) reduces plasma folate levels. }(\textbf{\textcolor{teal}{Supported}})         \\
Evidence 2 &    \textit{Twelve (63\%) of the 19 vitamin b12-deficient patients had elevated total homocysteine levels. (...) We conclude that there is a significant association of deficiencies of hb, iron, folic acid, and vitamin b12 and abnormally high blood homocysteine level with olp. }(\textbf{\textcolor{red}{Refuted}})           \\
                     \hline                                   \\
  (\textsc{PubMedQA})  & \textit{Wikipedia (Dense) }  \textit{PubMed (Dense)}  \\
  Claim: & \textbf{Does psychological distress predict disability?} (\textbf{\textcolor{teal}{Supported}})                  \\
  Evidence 1 & Mental distress can potentially lead to a change of behavior, affect a person's emotions in a negative way, and affect their relationships with the people around them. People under constant distress are more likely to become sick, mentally or physically. (\textbf{\textcolor{teal}{Supported}})            \\
  Evidence 2 &  The results of the mediation analysis suggest that approximately 30\% of the relationship between subacute pain and later disability is dependent on the level of patients' psychological distress. The finding that psychological distress only partially (30\%) mediated the pain-disability relationship indicates that other factors should also be explored.      (\textbf{\textcolor{red}{Refuted}})          \\
                     &                                    \\
(\textsc{HealthFC})   & \textit{Wikipedia (Sparse)}  \textit{Google snippets}  \\
Claim & \textbf{Does regular consumption of coffee increase the risk of heart disease such as heart attack or stroke?}     (\textbf{\textcolor{red}{Refuted}})                \\
Evidence 1 &    Drinking more than this amount actually increases the risk of heart disease, high blood pressure, atrial fibrillation, and stroke. (...) There is an increased risk of hypertriglyceridemia, cardiomyopathy, hypertension, and stroke if three or more standard drinks of alcohol are taken per day.       (\textbf{\textcolor{teal}{Supported}})        \\
Evidence 2 &         A meta-analysis concluded that coffee consumption did not provided any prophylactic effect on cardiovascular diseases but did not pose an increased risk either[...] \/\/ | The cohort study data suggest very little excess risk of coronary heart disease among habitual coffee drinkers. The case-controled data[...]   (\textbf{\textcolor{red}{Refuted}})    \\ 
                     &                    &                 \\
 (\textsc{CoVert})  & \textit{Alpaca (7B) }  \textit{Med-Alpaca (7B) }\\
 Claim & \textbf{Covid causes heart inflammation in like 70\% of people (including asymptomatic).  That seems like a high rate of heart inflammation!} (\textbf{\textcolor{red}{Refuted}})   \\
 Evidence 1 &    Yes, the claim is true. According to research, approximately 70\% of people with COVID-19 may develop inflammation of the heart, even if they do not have any symptoms of the virus. This is because the virus can cause long-term damage to the heart even if the person appears to be healthy.    (\textbf{\textcolor{teal}{Supported}}) \\
 Evidence 2       &      No, the claim is not true. Heart inflammation (myocarditis) is a rare condition that can be caused by a variety of factors, including viral infections. However, studies have found that the rate of myocarditis in patients with COVID-19 is similar to that seen in patients with other respiratory infections, such as the flu. While myocarditis can be a serious condition, it is not seen in the majority of patients with COVID-19. (\textbf{\textcolor{red}{Refuted}}) \\ \hline

          
\end{tabular}
\caption{\label{tab:comparison} Example claims and retrieved evidence from two different knowledge sources, or using two different retrieval techniques, where only one of them provided a correct final verdict.}
\end{table*}
%%%
\fi

%Finally, the comparison between the vanilla Alpaca model and the domain-specific Med-Alpaca provides a nice insight. It is visible that for all four datasets, Med-Alpaca was more successful in providing responses that end in a correct verdict. This is most notable for \textsc{CoVert}. This shows that fine-tuning of modern LLMs, which are instruction-tuned and conversational in nature, to a specific domain is indeed helpful in performing the performance for that domain. Still, these results have to be taken with the grain of salt since we only look at final verdict and disregard the actual quality of the generated responses in the numerical analysis. Manual inspection did uncover some responses which gave a correct verdict but contained hallucinated or irrelevant evidence to justify it. Therefore, a promising future endeavor could be retrieval-augmented medical assistant agents that combine the user-friendly generative responses with factual knowledge obtained from knowledge sources like PubMed or Wikipedia themselves. 

